KGValidator: A Framework for Automatic Validation of Knowledge Graph Construction

This study explores the use of Large Language Models (LLMs) for automatic evaluation of knowledge graph (KG) completion models. Historically, validating information in KGs has been a challenging task, requiring large-scale human annotation at prohibitive cost. With the emergence of general-purpose generative AI and LLMs, it is now plausible that human-in-the-loop validation could be replaced by a generative agent. We introduce a framework for consistency and validation when using generative models to validate knowledge graphs. Our framework is based upon recent open-source developments for structural and semantic validation of LLM outputs, and upon flexible approaches to fact checking and verification, supported by the capacity to reference external knowledge sources of any kind. The design is easy to adapt and extend, and can be used to verify any kind of graph-structured data through a combination of model-intrinsic knowledge, user-supplied context, and agents capable of external knowledge retrieval.

==> 3-1-b.tex <==
\begin{tikzpicture}[
    font=\ttfamily,
    bigbox/.style args={#1#2#3#4}{
        rounded corners, fill=#1, draw=gray, align=center, inner sep=#2, line width=0.1pt,
        append after command={
            \pgfextra{
                \node [rectangle, draw, fill=white, text width=#3, align=center, font=\scriptsize, above=-0.5mm of \tikzlastnode.north] {#4};
            }
        }
    },
    square_node/.style 2 args={
        rectangle, rounded corners, draw=none, fill=#1, 
        text width=#2, minimum height=#2, inner sep=1mm, align=center, font=\scriptsize,
    },
    square_node_header/.style 2 args={
        rectangle, rounded corners, draw=none, fill=#1, 
        text width=4.7cm, inner sep=1mm, align=left, font=\scriptsize,
        append after command={
            \pgfextra{
                \node [rectangle, draw, fill=white, text width=2.5cm, align=center, font=\scriptsize, above=-1mm of \tikzlastnode.north] {#2};
            }
        }
    },
    neuron/.style={circle, draw=none, fill=customRed, minimum size=0.25cm},
    pics/llm/.style={
        code={
            \begin{scope}[local bounding box=llm]
              % Draw the input layer
              \foreach \i in {1,...,3}
                \node[neuron] (-input-\i) at (0,\i*0.5-1) {};
              % Draw the hidden layer
              \foreach \i in {1,...,4}
                \node[neuron] (-hidden-\i) at (1,\i*0.5-1.25) {};
              % Draw the output neuron
              \node[neuron] (-output) at (1.75,0.05) {};
              % Draw the connections
              \foreach \i in {1,...,3}
                \foreach \j in {1,...,4}
                  \draw (-input-\i) -- (-hidden-\j);
              \foreach \i in {1,...,4}
                \draw (-hidden-\i) -- (-output);
            \end{scope}
        }
    }
]
    \tikzstyle{arrow} = [very thick,->,>=stealth, draw=black!50]
    \tikzstyle{arrow_dashed} = [very thick, dashed, ->, >=stealth, draw=black!50]
    
    % ------ NODES -----------

    % llm
    \pic [below=3cm of kg, xshift=-1cm] {llm};

    % bounding boxes
    \begin{scope}[on background layer]
        \node (external_llm_box) [bigbox={verylightgray}{2mm}{1cm}{LLM}, fit=(llm)] {};
    \end{scope};

    % data 1
    \node (unvalidated_triple1) [square_node_header={customLightBlue}{Unvalidated triple}, left=4cm of llm] {
        \{\\
        \ \ ``subject": ``anaheim\_ducks",\\
        \ \ ``relation": ``teamplaysport",\\
        \ \ ``object": ``football"\\
        \}\\
    };
    
    % data 1 - validated
    \node (validated_triple1) [square_node_header={customLightBlue}{Validated triple}, right=2cm of llm] {
        \{\\
        \ \ ``subject": ``anaheim\_ducks",\\
        \ \ ``relation": ``teamplaysport",\\
        \ \ ``object": ``football",\\
        \ \ \textcolor{red}{``is\_valid": False,}\\
        \ \ \textcolor{red}{``reason": ``The given context states that Anaheim Ducks are actually an ice hockey team."}\\
        \}    
    };
    
    % --- RAG Section ---

    % 1. Relevant documents
    
    % Place the stack's top document relative to 'llm'
    \node [draw, rectangle, fill=white, minimum width=2cm, minimum height=0.5cm, above=3cm of llm, label={[align=center, label distance=9mm]above:Relevant Fragments}] (relevant_docs) {};
    \draw[fill=white] ([yshift=-6mm]relevant_docs.south west) rectangle ++(2,0.5);
    \draw[fill=white] ([yshift=6mm]relevant_docs.south west) rectangle ++(2,0.5);
    \foreach \y in {0.3,0.5,0.9,1.1,1.5,1.7} {
        \draw ([xshift=2mm,yshift=-7.5mm+\y cm]relevant_docs.south west) -- ++(1.6,0);
    }

    % 2. Vector index
    % Placeholder for cylinder base position
    \node [left=2.5cm of relevant_docs] (vector_index) {};
    
    % Drawing the cylinder with adjustable height
    \begin{scope}[shift={(vector_index.center)}]
        % Define the cylinder dimensions
        \def\cylinderheight{1.5} % Adjustable height
        \def\cylinderradius{1}
    
        % Calculate half the cylinder height for positioning
        \pgfmathsetmacro\halfheight{\cylinderheight/2}
    
        % Cylinder top
        \filldraw[fill=customGrey] (0,-\halfheight) ellipse (\cylinderradius cm and 0.25cm);
    
        % Cylinder body
        % Adjusted to use \halfheight for dynamic height
        \fill[fill=customGrey] (-\cylinderradius cm,\halfheight) rectangle (\cylinderradius cm,-\halfheight);
    
        % Cylinder bottom
        % Adjusted to use -\halfheight for the bottom ellipse
        \filldraw[fill=customGrey] (0,\halfheight) ellipse (\cylinderradius cm and 0.25cm);
    
        % Optional: Cylinder top line for aesthetics
        \draw[dashed] (0,-\halfheight) ellipse (\cylinderradius cm and -0.25cm);
    \end{scope}
    
    % Label below the cylinder
    \node [align=center, above=11mm of vector_index] {Vector Index};
    
    % 3. Textual documents
    
    % Place the stack's top document relative to 'vector_index'
    \node [draw, rectangle, fill=white, minimum width=2cm, minimum height=1.5cm, left=2.8cm of vector_index, label={[align=center, label distance=5mm]above:Textual Documents}] (top_document) {};
    
    % Draw the second document in the stack (visually below the top document)
    \draw[fill=white] ([xshift=-2mm,yshift=2mm]top_document.south west) rectangle ++(2,1.5);
    
    % Draw the bottom document in the stack (visually below the second document)
    \draw[fill=white] ([xshift=-4mm,yshift=4mm]top_document.south west) rectangle ++(2,1.5);
    
    % Add text lines to the top document
    \foreach \y in {0.3,0.6,0.9,1.2} {
        \draw ([xshift=-2mm,yshift=0.4cm+\y cm]top_document.south west) -- ++(1.6,0);
    }    

    % ------ ARROWS -----------
    \draw [arrow] (unvalidated_triple1.east) -- (external_llm_box.west);
    \draw [arrow] (external_llm_box.east)  -- (validated_triple1.west);
    \draw [arrow] (top_document.east) -- ([xshift=-1cm]vector_index.center) node[midway, above, text width=2cm, align=center]{\scriptsize Chunking and encoding};
    \draw [arrow] ([xshift=1cm]vector_index.center) -- (relevant_docs);
    \draw [arrow] ([yshift=-8.5mm]relevant_docs.center) -- ([yshift=15mm]llm.center);
    \draw [arrow] (unvalidated_triple1.east) -| ([yshift=-1cm]vector_index.center) node[near end, above, text width=4cm, align=center]{\scriptsize \textbf{query:} string representation of triple};


\end{tikzpicture}

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
